SimNet: Accurate and High-Performance Computer Architecture Simulation using Deep Learning

While discrete-event simulators are essential tools for architecture research, design, and development, their practicality is limited by an extremely long time-to-solution for realistic applications under investigation. This work describes a concerted effort, where machine learning (ML) is used to accelerate discrete-event simulation. First, an ML-based instruction latency prediction framework that accounts for both static instruction properties and dynamic processor states is constructed. Then, a GPU-accelerated parallel simulator is implemented based on the proposed instruction latency predictor, and its simulation accuracy and throughput are validated and evaluated against a state-of-the-art simulator. Leveraging modern GPUs, the ML-based simulator outperforms traditional simulators significantly.

==> Makefile <==
MAINFILE = main.tex
ABSFILE = extended-abstract.tex

PDF = ${MAINFILE:%.tex=%.pdf} ${ABSFILE:%.tex=%.pdf}


all:  ${PDF}

%.pdf:  %.tex content/*.tex fig/* ref.bib
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM)  *.log *.aux *.pdf \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi


==> content/motivation.tex <==
\section{ML-based Simulation Framework}
\label{sect:mot}


\subsecspace
\subsection{Cycle-accurate Simulation Background}
\label{sect:mot:sim}

% explain performance simulation is eventually to predict instruction latency.
%Explain how simulators work, and simulating instruction latency is the core.

Computer architects use software cycle-accurate simulators extensively in the
early design stage because it often is prohibitively expensive to implement
real hardware prototypes in terms of both time and financial costs.
Simulators take one or a set of programs as their inputs.
%These input programs can be in the form of either execution traces (i.e.,
%trace-driven simulator) or binaries (i.e., execution-driven simulator).
The simulator explores the inputs instruction by instruction to simulate the
interaction between hardware and software, and it reports the performance
metrics and other statistics of interest as the output when all instructions
finish execution.

Internally, traditional simulators are composed of various software modules
that mimic the behavior of different hardware components.
Hardware system simulation is achieved by simulating individual
components within it and their interactions.
%We call these simulators, {\em component-centric}.

These traditional simulators are intrinsically difficult to parallelize because
of the heterogeneous nature of distinct components, the frequent interactions
between components, and the amount of available parallelism.
As a result, they cannot leverage modern high-performance accelerators such as
GPUs.


\subsecspace
\subsection{ML-based Instruction-centric Simulation}
\label{sect:mot:inst}

In this paper, we propose \simnet, an ML-based instruction-centric simulator.
Figure \ref{fig:mlsim} shows the overview of \simnet.
The key roles of \simnet{} are to 1) predict the latency of individual
instructions (Section \ref{sect:ml}) then 2) infer the program performance
based on these predicted latency (Section \ref{sect:sim}).
\simnet is able to improve simulation performance because, 1) it makes use of
ML models to abstract the simulated processor as a whole and eliminate the need
to simulate individual components, and 2) ML inferences are highly parallel and
modern accelerators are tailored for ML.

